Structured Reordering for Modeling Latent Alignments in Sequence Transduction

Despite success in many domains, neural models struggle in settings where train and test examples are drawn from different distributions. In particular, in contrast to humans, conventional sequence-to-sequence (seq2seq) models fail to generalize systematically, i.e., interpret sentences representing novel combinations of concepts (e.g., text segments) seen in training. Traditional grammar formalisms excel in such settings by implicitly encoding alignments between input and output segments, but are hard to scale and maintain. Instead of engineering a grammar, we directly model segment-to-segment alignments as discrete structured latent variables within a neural seq2seq model. To efficiently explore the large space of alignments, we introduce a reorder-first align-later framework whose central component is a neural reordering module producing {\it separable} permutations. We present an efficient dynamic programming algorithm performing exact marginal inference of separable permutations, and, thus, enabling end-to-end differentiable training of our model. The resulting seq2seq model exhibits better systematic generalization than standard models on synthetic problems and NLP tasks (i.e., semantic parsing and machine translation).

==> algorithms/inside.tex <==
\begin{algorithm}[t]
    \caption{The inside algorithm}
    \begin{algorithmic}[1]
        \Function{Inside}{score}
        \State initilalize $\beta[\dots]$ to 0
        \For{$i := 0$ \textbf{to} $n-1$} \Comment width-1 spans
            \State $\beta[X_i^{i+1}] = 1$ \Comment $\mathcal T$ rules with constant weight
        \EndFor
        \For{$w := 2$ \textbf{to} $n$} \Comment width of spans
            \For{$i := 0$ \textbf{to} $n - w$} \Comment start point
                \State $k := i + w$  \Comment end point
                \For{$j := i+1$ \textbf{to} $k-1$}
                   \State $\beta[X_i^k] += f_\phi(\mathcal{S}_{i,k,j}) \beta[X_i^j]\beta[X_{j}^{k}] $
                   \State $\beta[X_i^k] += f_\phi(\mathcal{I}_{i,k,j}) \beta[X_i^j]\beta[X_{j}^{k}] $
                \EndFor
            \EndFor
        \EndFor
        \State \Return $\beta[X_0^n]$
        \EndFunction
    \end{algorithmic}
    \label{algo:partition}
\end{algorithm}


==> algorithms/marginal_separate.tex <==
\begin{figure}[!t]
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[H]
    \caption{Computing the expected permutation matrix via dynamic programming}
    \begin{algorithmic}[1]
        % \Function{ComputeMarginal}{$p_m$}
        \For{$i := 1$ \textbf{to} $n$} % \Comment width-1 spans
            \State  $\mE_i^{i+1} = \bs 1$ 
        \EndFor
        \For{$w := 2$ \textbf{to} $n$} \Comment width of spans
            \For{$i := 1$ \textbf{to} $n - w + 1$} % \Comment start point
                \State $k := i + w$ % \Comment end point
                \For{$j := i+1$ \textbf{to} $k-1$}
                   \State $\mE_i^k \mathrel{+}= G_\phi(\mathcal{S}_{i,j,k}) (\mE_i^j \oplus \mE_j^k) $\label{algo:step-marginalize-1} % \Comment scalar-matrix multiplication
                   \State $\mE_i^k \mathrel{+}= G_\phi(\mathcal{I}_{i,j,k}) (\mE_i^j \ominus \mE_j^k) $\label{algo:step-marginalize-2} % \Comment scalar-matrix multiplication
                \EndFor
            \EndFor
        \EndFor
        \State \Return $\mE_1^{n+1}$
        %\EndFunction
    \end{algorithmic}
    \label{algo:marginal}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[H]
    \caption{Differentiable Sampling via dynamic programming}
    \begin{algorithmic}[1]
        % \Function{ComputeMarginal}{$p_m$}
        \For{$i := 1$ \textbf{to} $n$} % \Comment width-1 spans
            \State  $\mE_i^{i+1} = \bs 1$ 
        \EndFor
        \For{$w := 2$ \textbf{to} $n$}  \Comment width of spans
            \For{$i := 1$ \textbf{to} $n - w + 1$} % \Comment start point
                \State $k := i + w$  % \Comment end point
                \State $g \sim Gumbel(0)$  \Comment Gumbel noise
                \State $ \tilde G_\phi(R) = \softmax((G_\phi(R)+ g)/\tau)$\label{algo:step-sampling-1}
                \State $ \hat G_\phi(R) = \sargmax(\tilde G_\phi(R))$\label{algo:step-sampling-2}
                \For{$j := i+1$ \textbf{to} $k-1$}
                   \State $\mE_i^k \mathrel{+}= \hat G_\phi(\mathcal{S}_{i,j,k}) (\mE_i^j \oplus \mE_j^k) $ % \Comment scalar-matrix multiplication
                   \State $\mE_i^k \mathrel{+}= \hat G_\phi(\mathcal{I}_{i,j,k}) (\mE_i^j \ominus \mE_j^k) $  % \Comment scalar-matrix multiplication
                \EndFor
            \EndFor
        \EndFor
        \State \Return $\mE_1^{n+1}$ % \Comment $\tilde G_\phi$ for surrogate gradients
        % \EndFunction
    \end{algorithmic}
    \label{algo:sampling}
\end{algorithm}
\end{minipage}
\end{figure}

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We prove the correctness of Algorithm~\ref{algo:marginal-sampling} in the supplementary paper.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{They are included in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The way of constructing data splits are explained in Section~\ref{sec:experiment}. Details of neural models and hyperparameters are included in the supplementary paper.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{We report average accuracies in Table~\ref{tab:synthetic} as the standard errors of our models are very small (< 0.02). For brevity, 
    we conduct signficance tests in Table~\ref{tab:parsing} to highlight the results that are signficantly better than others.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{They are included in the supplementary paper.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The synthetic data used in Section~\ref{sec:diagnostic} is included in the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}

\begin{CJK*}{UTF8}{gbsn}
\input{tables/predictions}
\end{CJK*}

\paragraph{Efficiency}
A limitation of \modelname is the increased running time compared with the conventional seq2seq model. 
In semantic parsing, our model increases the training and inference 
time by a factor of 2; in machine translation, the factor is 4-6.
To address this, we have tried to introduce an autoregressive version of our model. Specifically, we replaced the module for monotonic alignment 
with Connectionist Temporal Classification (CTC)~\citep{graves2014towards}, 
which enjoys faster training and parallel decoding. In terms of decoding time, we found the resulting model 
is more efficient than the conventional seq2seq model in all our experiments.
However, CTC restricts the alignment to be many-to-one (i.e., input segment to output word) 
and cannot handle the cases where an input word is associated with an output segment. 
The many-to-one mapping suits the semantic parsing task well since the input sentences are 
usually longer than their corresponding programs. Indeed, we found the resulting model works well and 
even performs better than the Hard-\modelname in the semantic parsing experiments. However, this variant does not work as well in 
the machine translation task. We plan to explore ways of improving this variant in the future towards a more efficient seq2seq model with latent segment alignments.
%such as up-sampling input sentences~\cite{saharia2020non} to longer ones make this variant useful for machine translation.

% A further consideration is to investigate ways of coupling our model with current pre-trained 
% representations. Such representations, e.g., BERT and T5, are contextualized in the sense
% that the representation of a word or a segment is deeply influenced by its context. 
% In other words, implicit alignment (via self-attention) within a sequence is already baked into 
% the representations. Hence, modeling alignments directly on top of the contextualized 
% representations is undesirable. One potential direction is to inject inductive biases of 
% discrete alignments into pre-trained representations.

\paragraph{Other Applications}
The strong inductive bias introduced by modeling alignments in this work could be potentially
beneficial in low-resource and weakly-supervised settings, such as low-resource machine translation, 
weakly supervised semantic parsing where conventional seq2seq models usually do not perform well. 
We leave this line of exploration for future work.

==> sections/impact.tex <==
\section*{Broader Impact}

Talk about interpretability

==> sections/related_work.tex <==
\section{Additional Related Work}

%\paragraph{Reordering and Permutation} 

In traditional statistical machine translation (SMT), reorderings are typically handled by a distortion model~\citep[e.g.,][]{al2006distortion} in a pipeline manner.
\citet{neubig-etal-2012-inducing, nakagawa-2015-efficient} also use BTG for modeling reorderings,
but they assume the alignments have been produced on a preprocessing step, using an alignment tool~\cite{och-ney-2003-systematic}. Relying on these alignments, they induce reorderings. Inversely, we rely on latent reordering to induce 
the underlying alignments.
%or with synchronous production rules~\citep{chiang2005hierarchical}.
%

Reordering modules have been previously used in neural models, and can be assigned to the following two categories. 
%There exist two kinds of alternatives to our reordering module in previous work.
First, reordering components \citep{huang2017towards,chen2019neural} 
were proposed for neural machine translation. However, they are not structured or sufficiently constrained
in the sense that they may produce invalid reorderings (e.g., a word is likely to be moved to 
more than one new position). In contrast, our module is a principled way of dealing with latent reorderings.
Second, the generic permutations (i.e., one-to-one matchings), used previously in NLP~(e.g., \cite{lyu-titov-2018-amr}), do not suit our needs as they are defined in terms of tokens, rather than segments. They also require extra approximations to enable differentiable learning~\cite{mena2018learning}. We will compare with both classes of methods in our experiments.

%a) most algorithms for generic permutations operate on tokens, rather than segments~\citep[e.g.,][]{lyu-titov-2018-amr};
%b) the generic permutations rely on approximated methods, e.g., Sinkhorn operator for differentiable 
%learning~\citep{mena2018learning}, making the training process less sound. We will compare our model
%with both kinds of methods in our experiments. 
%

% Another important distinction is that in our algorithm separable permutations 
% can preserve segments by the construction of binary trees, whereas, making them not suitable to model segment-level alignments.
% As opposed to modeling all possible segment alignments in one step, this is more desirable 
% as both steps permit efficient inference (i.e., MAP and 
% marginal inference, as we will discuss later) that are required for training. 
% In both permutations and monotonic alignments, the segmentations are unknown and treated as discrete random variables.

%\paragraph{Grammar-based Models} 
%Grammar formalisms such as Combinatorial Categorical Grammar (CCG)~\cite{steedman2000syntactic}
%and Synchronous Context-free Grammar (SCFG) were shown beneficial in
%traditional SMT~\cite{chiang2005hierarchical} and semantic parsing~\cite{zettlemoyer2012learning,wong-mooney-2006-learning}.
%In the neural era, these works have gained renewed interests due to accumulating evidence 
%showing that current seq2seq models cannot generalize systematically.  
%Recent attempts~\cite{herzig2020span,shaw2020compositional} that incorporate
%grammar-based structures into neural parser for modeling tree-level correspondences.
%However, they are specialized for semantic parsing where output (i.e., programs) have natural known
%tree structures. Our work follows the same spirit as these work
%but does not require that output has grammar.

% to take advantage of both grammar-based and seq2seq models.
% In contrast, our model does not require that output have tree structures, 
% implying that it can be applied to more general tasks beyond 
% semantic parsing. 

==> tables/nmt_with_dev.tex <==
\begin{table}
    \center
    \scalebox{0.9}{
    \begin{tabular}{ l|cccc|cccc } 
        \toprule
        & \multicolumn{4}{c|}{\textbf{EN-JA}} & \multicolumn{4}{c}{\textbf{ZH-EN}} \\
        \cmidrule(lr){2-5}
        \cmidrule(lr){6-9}
        & \multicolumn{2}{c}{\textsc{IID}} & \multicolumn{2}{c|}{\textsc{Len}} & \multicolumn{2}{c}{\textsc{IID}} & \multicolumn{2}{c}{\textsc{Len}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
        & Dev & Test & Dev & Test & Dev & Test & Dev & Test  \\
        \midrule
        % Previous work \cite{chousa2019simultaneous} & - & 34.53 \\
        %\hline
        Seq2Seq & 36.5 & 35.6 & 25.6 & 25.3 & 22.5 & 21.4 & 18.4 & 18.1 \\ 
        SSNT~\citep{yu2016online}  & 36.7 & 36.3 & 26.8 & 26.5 & 22.3 & 20.5 & 17.7 & 17.3 \\
        SSNT + {\small Local Reordering}~\citep{huang2017towards} & 37.0 & 36.0 & 26.3 & 27.1 & 22.7 & 21.8 & 18.3 & 17.8 \\ 
        \hdashline
        Soft-\modelname & 37.4 & 36.6 &  27.3 & 27.5 & \bf{23.8} & 22.3 & 18.8 & 18.7 \\
        Hard-\modelname  & \bf{38.4} & \bf{37.4} & \bf{28.3} & \bf{28.7} & 23.6 & \bf{22.6} & \bf{19.6} & \bf{19.5}  \\
        \bottomrule
       \end{tabular}
    }
    \caption{BLEU scores on the EN-JA and ZH-EN translation tasks.}
    \label{tab:nmt}
\end{table}
